A Neural Network Approach to Efficient Valuation of Large Portfolios of Variable Annuities

Managing and hedging the risks associated with Variable Annuity (VA) products require intraday valuation of key risk metrics for these products. The complex structure of VA products and computational complexity of their accurate evaluation have compelled insurance companies to adopt Monte Carlo (MC) simulations to value their large portfolios of VA products. Because the MC simulations are computationally demanding, especially for intraday valuations, insurance companies need more efficient valuation techniques. Recently, a framework based on traditional spatial interpolation techniques has been proposed that can significantly decrease the computational complexity of MC simulation (Gan and Lin, 2015). However, traditional interpolation techniques require the definition of a distance function that can significantly impact their accuracy. Moreover, none of the traditional spatial interpolation techniques provide all of the key properties of accuracy, efficiency, and granularity (Hejazi et al., 2015). In this paper, we present a neural network approach for the spatial interpolation framework that affords an efficient way to find an effective distance function. The proposed approach is accurate, efficient, and provides an accurate granular view of the input portfolio. Our numerical experiments illustrate the superiority of the performance of the proposed neural network approach compared to the traditional spatial interpolation schemes.

==> accuracy.tex <==
\subsection{Accuracy}\label{sec:accuracy}
The accuracy results of Table \ref{tb:rel_err1} may misleadingly 
suggest that the Kriging method with the Spherical variogram model is 
always capable of providing very accurate interpolations. In the 
experiments of this section, we provide results on the accuracy of 
different methods that contradicts this hypothesis. 

For our experiments in this section, we replicated the experiments 
of Section \ref{sec:performance}  with sets of representative contracts 
that are produced from the set of representative contracts in Section \ref{sec:performance} 
by removing $100$, $200$, $400$, $600$ and $800$ \ac{VA} contracts 
at random. Table \ref{tb:rel_err4} presents the mean and the standard deviation 
of the relative error, in estimation of the delta value of the 
\ac{VA} portfolio, for each method in these experiments. 
The results of Table \ref{tb:rel_err4} show high variance values for the  
accuracy of the Kriging methods, 
which contradicts our hypothesis. Another interesting observation 
is that the IDW methods and the RBF 
methods with a Gaussian kernel, in comparison to the Kriging methods, 
have a lower variance value for the relative error. 


\begin{table}[!bt]
 \centering
 \begin{tabular}{|l|l|l|}
  \hline
  Method & Mean (\%) & STD (\%)\\ 
  \hline
  Kriging (Spherical) & $0.47$ & $1.76$\\ 
  \hline
  Kriging (Exponential) & $-0.58$ & $2.19$\\
  \hline 
  Kriging (Guassian) & $1109.02$ & $3289.81$\\
  \hline
  IDW (p = 1) & $9.14$ & $1.75$\\
  \hline 
  IDW (p = 10) & $13.14$ & $0.42$\\
  \hline
  IDW (p = 100) & $12.06$ & $0.23$\\ 
  \hline 
  RBF (Gaussian, $\epsilon = 1$) & $-1.78$ & $0.48$\\
  \hline
  RBF (Gaussian, $\epsilon = 10$) & $38.87$ & $1.42$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 1$) & $-58.65$ & $16.84$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 10$) & $-9.15$ & $3.56$\\
  \hline
 \end{tabular}
 \caption{Mean and standard deviation of relative error in estimation of delta value via each method.}
 \label{tb:rel_err4}
\end{table}

